H2Learn: High-Efficiency Learning Accelerator for High-Accuracy Spiking Neural Networks

Although spiking neural networks (SNNs) take benefits from the bio-plausible neural modeling, the low accuracy under the common local synaptic plasticity learning rules limits their application in many practical tasks. Recently, an emerging SNN supervised learning algorithm inspired by backpropagation through time (BPTT) from the domain of artificial neural networks (ANNs) has successfully boosted the accuracy of SNNs and helped improve the practicability of SNNs. However, current general-purpose processors suffer from low efficiency when performing BPTT for SNNs due to the ANN-tailored optimization. On the other hand, current neuromorphic chips cannot support BPTT because they mainly adopt local synaptic plasticity rules for simplified implementation. In this work, we propose H2Learn, a novel architecture that can achieve high efficiency for BPTT-based SNN learning which ensures high accuracy of SNNs. At the beginning, we characterized the behaviors of BPTT-based SNN learning. Benefited from the binary spike-based computation in the forward pass and the weight update, we first design lookup table (LUT) based processing elements in Forward Engine and Weight Update Engine to make accumulations implicit and to fuse the computations of multiple input points. Second, benefited from the rich sparsity in the backward pass, we design a dual-sparsity-aware Backward Engine which exploits both input and output sparsity. Finally, we apply a pipeline optimization between different engines to build an end-to-end solution for the BPTT-based SNN learning. Compared with the modern NVIDIA V100 GPU, H2Learn achieves 7.38x area saving, 5.74-10.20x speedup, and 5.25-7.12x energy saving on several benchmark datasets.

==> text/index.tex <==
\clearpage
\section{Index Sheet for Revision}

\textit{The revision texts are in \todob{blue}. Moreover, the indexes of reviewers' questions are in \todor{red} (for example, A3 means the revision for the third question of Reviewer\#3)}.

\vspace{25pt}

\subsection{Common Questions}

[CQ1] [@Reviewer-A/C] 

[Why BPTT-based SNN training and accelerator] 

\textit{Revision: start of Sec. III, Sec. III.B with added Tab. II.}

\vspace{5pt}

[CQ2] [@Reviewer-A/D/E] 

[Batch size setting]

\textit{Revision: end of Sec. IV.}

\vspace{5pt}

[CQ3] [@Reviewer-B/D] 

[Baseline details]

\textit{Revision: start of Sec. V.B.}

\vspace{25pt}

\subsection{Reviewer Questions}

[A1-CQ1] [Why GPU not efficient enough and the value of efficiency increase] 

\textit{Revision: start of Sec. III, Sec. III.B with added Tab. II.}

\vspace{5pt}

[A2-CQ2] [Batch size setting on GPU]

\textit{Revision: end of Sec. IV.}

\vspace{25pt}

[B1-CQ3] [Baseline details]

\textit{Revision: start of Sec. V.B.}

\vspace{5pt}

[B2] [How to model SpinalFlow]

\textit{Revision: end of Sec. V.A}

\vspace{5pt}

[B3] [Target scenario with a 20W accelerator]

\textit{Revision: end of Sec. V.A}

\vspace{25pt}

[C1-CQ1] [Why BPTT-based SNN training accelerator]

\textit{Revision: start of Sec. III, Sec. III.B with added Tab. II.}

\vspace{5pt}

[C2] [Other operations beyond convolution]

\textit{Revision: start of Sec. IV.B.}

\vspace{5pt}

[C3] [SNNs vs. ANNs]

\textit{Revision: start of Sec. I, start of Sec. III.}

\vspace{25pt}

[D1] [Novelty of LUT design and LUT details]

\textit{Revision: Sec. IV.B.1), Sec. V.B.1), Fig. 11, Fig. 12.}

\vspace{5pt}

[D2] [Meaning of cm\_n]

\textit{Revision: Tab. III.}

\vspace{5pt}


[D3] [How to do accumulation and what’s the accumulation data type]

\textit{Revision: Sec. IV.B.1).}

\vspace{5pt}

[D4] [Neuron ID]

\textit{Revision: Sec. IV.B.3).}

\vspace{5pt}

[D5-CQ2] [Batch size setting]

\textit{Revision: end of Sec. IV.}

\vspace{5pt}

[D6] [Off-chip memory setting]

\textit{Revision: end of Sec. V.C.}

\vspace{5pt}

[D7-CQ3] [Accelerator baseline]

\textit{Revision: start of Sec. V.B.}

\vspace{5pt}

[D8] [GPU baseline]

\textit{Revision: end of Sec. V.C.}

\vspace{5pt}

[D9] [Absolute power consumption in Fig.16]

\textit{Revision: Fig.16.}

\vspace{5pt}

[D10] [Outer control and loss computation and \#iteration determination]

\textit{Revision: end of Sec. IV.C.1).}

\vspace{25pt}

[E1] [Why SNN-BPTT costly]

\textit{Revision: Sec. III.C.}

\vspace{5pt}

[E2] [What are invalid neurons]

\textit{Revision: end of Sec. IV.A. }

\vspace{5pt}

[E3] [Regarding three DRAM or DRAM sticks]

\textit{Revision: start of Sec. IV.C.1).}

\vspace{5pt}

[E4] [Optimal setting in Fig.14]

\textit{Revision: Sec. V.C.}

\vspace{5pt}

[E5] [Earlier citation of LUT optimal setting]

\textit{Revision: Sec. IV.B.1).}

\vspace{5pt}

[E6-CQ2] [Batch setting and sub-batch pipeline]

\textit{Revision: end of Sec. IV.}

\vspace{5pt}

[E7] [Relative improvement vs. parallelism]

\textit{Revision: Fig. 12, Fig. 13.}

\vspace{5pt}

[E8] [Micro-architecture details]

\textit{Revision: Fig. 5, Fig. 8.}





